TrustSQL: Benchmarking Text-to-SQL Reliability with Penalty-Based Scoring

Text-to-SQL enables users to interact with databases using natural language, simplifying the retrieval and synthesis of information. Despite the remarkable success of large language models (LLMs) in translating natural language questions into SQL queries, widespread deployment remains limited due to two primary challenges. First, the effective use of text-to-SQL models depends on users' understanding of the model's capabilities-the scope of questions the model can correctly answer. Second, the absence of abstention mechanisms can lead to incorrect SQL generation going unnoticed, thereby undermining trust in the model's output. To enable wider deployment, it is crucial to address these challenges in model design and enhance model evaluation to build trust in the model's output. To this end, we introduce TrustSQL, a novel comprehensive benchmark designed to evaluate text-to-SQL reliability-defined as a model's ability to correctly handle any type of input question by generating correct SQL queries for feasible questions and abstaining from generating infeasible ones (e.g., due to schema incompatibility or functionalities beyond SQL). We evaluate existing methods using a novel penalty-based scoring metric with two modeling approaches: (1) pipeline-based methods combining SQL generators with infeasible question detectors and SQL error detectors for abstention; and (2) unified methods using a single model for the entire task. Our experimental results reveal that achieving high scores under severe penalties requires significant effort and provide a new perspective on developing text-to-SQL models for safer deployment. TrustSQL is available at https://github.com/glee4810/TrustSQL.

==> prompts/classifier_prompt_cross.tex <==
\textcolor{blue}{CREATE TABLE} artist ( \\ 
artist\_id \textcolor{blue}{number}  , \\ 
name \textcolor{blue}{text}  , \\ 
country \textcolor{blue}{text}  , \\ 
year\_join \textcolor{blue}{number}  , \\ 
age \textcolor{blue}{number}  , \\ 
\textcolor{blue}{primary key} ( artist\_id ) \\ 
) \\ 
/* \\ 
Columns in artist and 3 examples in each column: \\ 
Artist\_ID: 1, 2, 3 \\ 
Name: Vijay Singh, John Daly, Paul Azinger \\ 
Country: Fiji, United States, United States \\ 
Year\_Join: 1998, 1991, 1993 \\ 
Age: 45, 46, 47 \\ 
*/ \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} exhibition ( \\ 
exhibition\_id \textcolor{blue}{number}  , \\ 
year \textcolor{blue}{number}  , \\ 
theme \textcolor{blue}{text}  , \\ 
artist\_id \textcolor{blue}{number}  , \\ 
ticket\_price \textcolor{blue}{number}  , \\ 
\textcolor{blue}{primary key} ( exhibition\_id ) , \\ 
\textcolor{blue}{foreign key} ( artist\_id ) \textcolor{blue}{references}  artist ( artist\_id ) \\ 
) \\ 
/* \\ 
 \\ 
Columns in exhibition and 3 examples in each column: \\ 
Exhibition\_ID: 1, 2, 3 \\ 
Year: 2004, 2005, 2006 \\ 
Theme: Santa Claus, Christmas stocking, Santa Claus and Rudolph the Red-Nosed Reindeer \\ 
Artist\_ID: 1, 2, 4 \\ 
Ticket\_Price: 19.95, 19.95, 14.95 \\ 
*/ \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} exhibition\_record ( \\ 
exhibition\_id \textcolor{blue}{number}  , \\ 
date \textcolor{blue}{text}  , \\ 
attendance \textcolor{blue}{number}  , \\ 
\textcolor{blue}{primary key} ( exhibition\_id ) , \\ 
\textcolor{blue}{foreign key} ( exhibition\_id ) \textcolor{blue}{references}  exhibition ( exhibition\_id ) \\ 
) \\ 
/* \\ 
Columns in exhibition\_record and 3 examples in each column: \\ 
Exhibition\_ID: 1, 1, 1 \\ 
Date: December 2, December 5, December 7 \\ 
Attendance: 965, 1098, 2983 \\ 
*/ \\ 
 \\ 
Please classify the following sentence into either answerable or unanswerable. Answer me with "answerable" or "not\_answerable". \\ 
 \\ 
Question: how many staff members work at the top-rated restaurant in alameda ? \\ 
Answer: not\_answerable \\ 
 \\ 
Question: who is the original singer for chicago? \\ 
Answer: not\_answerable \\ 
 \\ 
Question: What are the names of all songs in English? \\ 
Answer: answerable \\ 
 \\ 
Question: How many tracks does each genre have and what are the names of the top 5? \\ 
Answer: answerable 
\\ 
\\
\\
\{omitted\}
\\
\\
\\
\textcolor{blue}{CREATE TABLE} artist ( \\ 
artist\_id \textcolor{blue}{number}  , \\ 
artist \textcolor{blue}{text}  , \\ 
age \textcolor{blue}{number}  , \\ 
famous\_title \textcolor{blue}{text}  , \\ 
famous\_release\_date \textcolor{blue}{text}  , \\ 
\textcolor{blue}{primary key} ( artist\_id ) \\ 
) \\ 
/* \\ 
Columns in artist and 3 examples in each column: \\ 
Artist\_ID: 1, 2, 3 \\ 
Artist: Gorgoroth, Ophiolatry, Ophiolatry \\ 
Age: 34, 35, 22 \\ 
Famous\_Title: Bergen 1996, Transmutation, Antievangelistical Process (re-release) \\ 
Famous\_Release\_date: November 2007, January 21, 2008, 2009 \\ 
*/ \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} volume ( \\ 
volume\_id \textcolor{blue}{number}  , \\ 
volume\_issue \textcolor{blue}{text}  , \\ 
issue\_date \textcolor{blue}{text}  , \\ 
weeks\_on\_top \textcolor{blue}{number}  , \\ 
song \textcolor{blue}{text}  , \\ 
artist\_id \textcolor{blue}{number}  , \\ 
\textcolor{blue}{primary key} ( volume\_id ) , \\ 
\textcolor{blue}{foreign key} ( artist\_id ) \textcolor{blue}{references}  artist ( artist\_id ) \\ 
) \\ 
/* \\ 
Columns in volume and 3 examples in each column: \\ 
Volume\_ID: 1, 2, 3 \\ 
Volume\_Issue: 45:14 §, 45:15, 45:16 \\ 
Issue\_Date: 27 December 1986 - 10 January, 17 January, 24 January \\ 
Weeks\_on\_Top: 3.0, 1.0, 1.0 \\ 
Song:  The Way,  Everybody Have Fun Tonight ,  Walk Like an Egyptian  \\ 
Artist\_ID: 1, 2, 1 \\ 
*/ \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} music\_festival ( \\ 
id \textcolor{blue}{number}  , \\ 
music\_festival \textcolor{blue}{text}  , \\ 
date\_of\_ceremony \textcolor{blue}{text}  , \\ 
category \textcolor{blue}{text}  , \\ 
volume \textcolor{blue}{number}  , \\ 
result \textcolor{blue}{text}  , \\ 
\textcolor{blue}{primary key} ( id ) , \\ 
\textcolor{blue}{foreign key} ( volume ) \textcolor{blue}{references}  volume ( volume\_id ) \\ 
) \\ 
/* \\ 
Columns in music\_festival and 3 examples in each column: \\ 
ID: 1, 2, 3 \\ 
Music\_Festival: 34th England Academy Prize, 34th Japan Academy Prize, 34th European Academy Prize \\ 
Date\_of\_ceremony: 18 February 2011, 18 February 2011, 18 February 2011 \\ 
Category: Best Song, Best Lyrics, Best Song \\ 
Volume: 1, 2, 3 \\ 
Result: Nominated, Nominated, Awarded \\ 
*/ \\ 
 \\ 
Please classify the following sentence into either answerable or unanswerable. Answer me with "answerable" or "not\_answerable". \\ 
 \\ 
Question: Find the number of users in each role. \\ 
Answer: answerable \\ 
 \\ 
Question: how many manufacturers of whiskey are there in the us? \\ 
Answer: not\_answerable \\ 
 \\ 
Question: How many vehicle in total? \\ 
Answer: answerable \\ 
 \\ 
Question: who are morgan's co-stars? \\ 
Answer: not\_answerable \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} stadium ( \\ 
stadium\_id \textcolor{blue}{number}  , \\ 
location \textcolor{blue}{text}  , \\ 
name \textcolor{blue}{text}  , \\ 
capacity \textcolor{blue}{number}  , \\ 
highest \textcolor{blue}{number}  , \\ 
lowest \textcolor{blue}{number}  , \\ 
average \textcolor{blue}{number}  , \\ 
\textcolor{blue}{primary key} ( stadium\_id ) \\ 
) \\ 
/* \\ 
Columns in stadium and 3 examples in each column: \\ 
Stadium\_ID: 1, 2, 3 \\ 
Location: Raith Rovers, Ayr United, East Fife \\ 
Name: Stark's Park, Somerset Park, Bayview Stadium \\ 
Capacity: 10104, 11998, 2000 \\ 
Highest: 4812, 2363, 1980 \\ 
Lowest: 1294, 1057, 533 \\ 
Average: 2106, 1477, 864 \\ 
*/ \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} singer ( \\ 
singer\_id \textcolor{blue}{number}  , \\ 
name \textcolor{blue}{text}  , \\ 
country \textcolor{blue}{text}  , \\ 
song\_name \textcolor{blue}{text}  , \\ 
song\_release\_year \textcolor{blue}{text}  , \\ 
age \textcolor{blue}{number}  , \\ 
is\_male others , \\ 
\textcolor{blue}{primary key} ( singer\_id ) \\ 
) \\ 
/* \\ 
Columns in singer and 3 examples in each column: \\ 
Singer\_ID: 1, 2, 3 \\ 
Name: Joe Sharp, Timbaland, Justin Brown \\ 
Country: Netherlands, United States, France \\ 
Song\_Name: You, Dangerous, Hey Oh \\ 
Song\_release\_year: 1992, 2008, 2013 \\ 
Age: 52, 32, 29 \\ 
Is\_male: F, T, T \\ 
*/ \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} concert ( \\ 
concert\_id \textcolor{blue}{number}  , \\ 
concert\_name \textcolor{blue}{text}  , \\ 
theme \textcolor{blue}{text}  , \\ 
stadium\_id \textcolor{blue}{text}  , \\ 
year \textcolor{blue}{text}  , \\ 
\textcolor{blue}{primary key} ( concert\_id ) , \\ 
\textcolor{blue}{foreign key} ( stadium\_id ) \textcolor{blue}{references}  stadium ( stadium\_id ) \\ 
) \\ 
/* \\ 
Columns in concert and 3 examples in each column: \\ 
concert\_ID: 1, 2, 3 \\ 
concert\_Name: Auditions, Super bootcamp, Home Visits \\ 
Theme: Free choice, Free choice 2, Bleeding Love \\ 
Stadium\_ID: 1, 2, 2 \\ 
Year: 2014, 2014, 2015 \\ 
*/ \\ 
 \\ 
\textcolor{blue}{CREATE TABLE} singer\_in\_concert ( \\ 
concert\_id \textcolor{blue}{number}  , \\ 
singer\_id \textcolor{blue}{text}  , \\ 
\textcolor{blue}{primary key} ( concert\_id ) , \\ 
\textcolor{blue}{foreign key} ( singer\_id ) \textcolor{blue}{references}  singer ( singer\_id ) , \\ 
\textcolor{blue}{foreign key} ( concert\_id ) \textcolor{blue}{references}  concert ( concert\_id ) \\ 
) \\ 
/* \\ 
Columns in singer\_in\_concert and 3 examples in each column: \\ 
concert\_ID: 1, 1, 1 \\ 
Singer\_ID: 2, 3, 5 \\ 
*/ \\ 
 \\ 
Please classify the following sentence into either answerable or unanswerable. Answer me with "answerable" or "not\_answerable". \\ 
 \\ 
Question: How many singers do we have? \\ 
Answer: \\ 


==> prompts/classifier_prompt_single.tex <==
\textcolor{blue}{\textcolor{blue}{CREATE TABLE}} aircraft (\\
aircraft\_code \textcolor{blue}{text}  , \\
aircraft\_description \textcolor{blue}{text}  , \\ 
manufacturer \textcolor{blue}{text}  , \\ 
basic\_type \textcolor{blue}{text}  , \\ 
engines \textcolor{blue}{number}  , \\ 
propulsion \textcolor{blue}{text}  , \\ 
wide\_body \textcolor{blue}{text}  , \\ 
wing\_span \textcolor{blue}{number}  , \\ 
length \textcolor{blue}{number}  , \\ 
weight \textcolor{blue}{number}  , \\ 
capacity \textcolor{blue}{number}  , \\ 
pay\_load \textcolor{blue}{number}  ,  \\ 
cruising\_speed \textcolor{blue}{number}  , \\
range\_miles \textcolor{blue}{number}  , \\
pressurized \textcolor{blue}{text}  \\
) 
/* \\
Columns in aircraft and 3 examples in each column: \\ 
aircraft\_code: 100, 146, 310\\
aircraft\_description: fokker 100, british aerospace 146 (all series), airbus industrie a310 (all series) \\
manufacturer: fokker, british aerospace, airbus industrie \\
basic\_type: 100, 146, a310 \\
engines: 2, 4, 2 \\
propulsion: jet, jet, jet \\
wide\_body: no, no, yes\\
wing\_span: 92, 86, 144\\
length: 117, 102, 153\\
weight: 95000, 93000, 330695\\
capacity: 119, 112, 280\\
pay\_load: 27305.0, 23100.0, 79560.0\\
cruising\_speed: nan, 440.0, nan\\
range\_miles: 1502.0, 1924.0, 5113.0\\
pressurized: yes, yes, yes\\
*/
\\ 
\\
\\
\{omitted\}
\\
\\
\\
\textcolor{blue}{CREATE TABLE} time\_zone ( \\
time\_zone\_code \textcolor{blue}{text}  , \\
time\_zone\_name \textcolor{blue}{text}  , \\
hours\_from\_gmt \textcolor{blue}{number}  \\
)
\\
/*
Columns in time\_zone and 3 examples in each column: \\
time\_zone\_code: cst, est, mst \\
time\_zone\_name: central standard time, eastern standard time, mountain standard time \\
hours\_from\_gmt: -6, -5, -7 \\
*/
\\
\\
Please classify the following sentence into either answerable or unanswerable. Answer me with "answerable" or "not\_answerable".
\\\\
Question: can you specify the airline that has the most number of flights delayed
\\
Answer: not\_answerable
\\
\\
Question: list all flights arriving at mke \\
Answer: answerable
\\
\\
Question: list all the arriving flights at mke
\\
Answer: answerable
\\
\\
Question: may i know the airline with the most frequent delayed flights
\\
Answer: not\_answerable
\\
\\
Question: list all the flights that arrive at mke airport
\\
Answer: answerable
\\
\\
Question: list all the flights that arrive at mke from various cities
\\
Answer: answerable
\\
\\
Question: which airline has been operating the newest time
\\
Answer: not\_answerable
\\\\
Question: could you inform me about the airline that records the highest number of delayed flights
\\
Answer: not\_answerable
\\
\\
Question: list all the flights that arrive at mke
\\
Answer:




==> prompts/error_prompt.tex <==
% \textcolor{blue}{\#\#\#\# Based on the question and predicted SQL, are you sure the SQL below is correct? If you consider the SQL is correct, answer me with 'correct'. If not, answer me with 'incorrect'. Only output your response without explanation.} \\

% Table Other\_Available\_Features, columns = [feature\_id,feature\_type\_code,feature\_name,\\ feature\_description] \\
% Table Other\_Property\_Features, columns = [property\_id,feature\_id,property\_feature\_description] \\
% Table Properties, columns = [property\_id,property\_type\_code,date\_on\_market,date\_sold,\\ property\_name,property\_address,room\_count,vendor\_requested\_price,buyer\_offered\_price,\\ agreed\_selling\_price,apt\_feature\_1,apt\_feature\_2,apt\_feature\_3,fld\_feature\_1,fld\_feature\_2,\\ fld\_feature\_3,hse\_feature\_1,hse\_feature\_2,hse\_feature\_3,oth\_feature\_1,oth\_feature\_2,oth\_feature\_3, \\ shp\_feature\_1,shp\_feature\_2,shp\_feature\_3,other\_property\_details] \\
% Table Ref\_Feature\_Types, columns = [feature\_type\_code,feature\_type\_name] \\ 
% Table Ref\_Property\_Types, columns = [property\_type\_code,property\_type\_description] \\
% Foreign\_keys = [Other\_Available\_Features.feature\_type\_code = \\ Ref\_Feature\_Types.feature\_type\_code,Properties.property\_type\_code \\ = Ref\_Property\_Types.property\_type\_code,Other\_Property\_Features.property\_id = \\Properties.property\_id,Other\_Property\_Features.feature\_id = Other\_Available\_Features.feature\_id] \\
% Primary\_keys = [Ref\_Feature\_Types.feature\_type\_code,Ref\_Property\_Types.property\_type\_code, \\ Other\_Available\_Features.feature\_id,Properties.property\_id] \\

% \textcolor{blue}{Question:} Show the property type descriptions of properties belonging to that code. \\
% \textcolor{blue}{Predicted SQL:} SELECT property\_type\_description FROM Ref\_Property\_Types WHERE property\_type\_code = [property code]



\#\#\#\# Based on the question and predicted SQL, are you sure the SQL below is correct? If you consider the SQL is correct, answer me with 'correct'. If not, answer me with 'incorrect'. Only output your response without explanation. \\

Table Other\_Available\_Features, columns = [feature\_id,feature\_type\_code,feature\_name,\\ feature\_description] \\
Table Other\_Property\_Features, columns = [property\_id,feature\_id,property\_feature\_description] \\
Table Properties, columns = [property\_id,property\_type\_code,date\_on\_market,date\_sold,\\ property\_name,property\_address,room\_count,vendor\_requested\_price,buyer\_offered\_price,\\ agreed\_selling\_price,apt\_feature\_1,apt\_feature\_2,apt\_feature\_3,fld\_feature\_1,fld\_feature\_2,\\ fld\_feature\_3,hse\_feature\_1,hse\_feature\_2,hse\_feature\_3,oth\_feature\_1,oth\_feature\_2,oth\_feature\_3, \\ shp\_feature\_1,shp\_feature\_2,shp\_feature\_3,other\_property\_details] \\
Table Ref\_Feature\_Types, columns = [feature\_type\_code,feature\_type\_name] \\ 
Table Ref\_Property\_Types, columns = [property\_type\_code,property\_type\_description] \\
Foreign\_keys = [Other\_Available\_Features.feature\_type\_code = \\ Ref\_Feature\_Types.feature\_type\_code,Properties.property\_type\_code \\ = Ref\_Property\_Types.property\_type\_code,Other\_Property\_Features.property\_id = \\Properties.property\_id,Other\_Property\_Features.feature\_id = Other\_Available\_Features.feature\_id] \\
Primary\_keys = [Ref\_Feature\_Types.feature\_type\_code,Ref\_Property\_Types.property\_type\_code, \\ Other\_Available\_Features.feature\_id,Properties.property\_id] \\

Question: Show the property type descriptions of properties belonging to that code. \\
Predicted SQL: SELECT property\_type\_description FROM Ref\_Property\_Types WHERE property\_type\_code = [property code]

==> table/debug_thing.tex <==


\begin{table*}[t!]
\caption{Model comparison in TrustSQL involving both feasible and infeasible questions evaluated in $\phi_{_{0}}$, $\phi_{_{10}}$, and $\phi_{_{N}}$. AT, AD, EH, and SP refer to ATIS, Advising, EHRSQL, and Spider, respectively. \textsc{Abstain-All} blindly abstains from predicting all input questions, reflecting the ratio of infeasible questions. All in \% for readability.}
\centering
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{width=\textwidth,center}
\large
\begin{tabular}{ccccccccccccccc}
\hline

% \cmidrule(lr){4-15}

\multicolumn{3}{c}{}
& \multicolumn{4}{c}{$\phi_{0}$}
& \multicolumn{4}{c}{$\phi_{10}$}
& \multicolumn{4}{c}{$\phi_{N}$} \\ % [-0.5ex]

\cmidrule(lr){4-7}
\cmidrule(lr){8-11}
\cmidrule(lr){12-15}

& &
& AT & AD & EH & SP
& AT & AD & EH & SP
& AT & AD & EH & SP \\ % [-0.1ex]

% & &
% & Spider & ATIS & Advising & EHRSQL
% & Spider & ATIS & Advising & EHRSQL
% & Spider & ATIS & Advising & EHRSQL \\ % [-0.1ex]

% \hline
\hline

\multicolumn{2}{c}{} & \textsc{Abstain-All}
& 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 \\

\hline
\hline
\cellcolor{white!50} \multirow{7}{*}{Open}

& \multirow{3}{*}{Pipeline}
& \textsc{CLS$_M$} → \textsc{T5}
& 55.7 & 48.1 & 62.7 & \underline{61.1} & -160.7 & -154.5 & -60.4 & -304.2 & -20.5K & -21.6K & -22.9K & -38.4K\\

& & \textsc{T5} → \textsc{Error$_{M}$} 
& \textbf{73.0} & 73.8 & 75.5 & 60.3 & -59.3 & -133.5 & -115.6 & -121.8 & -12.5K & -22.0K & -35.6K & -19.1K
 \\

& & \textsc{CLS$_M$} → \textsc{T5} → \textsc{Error$_M$}
& 64.3 & 58.9 & 66.5 & \textbf{64.3} & \underline{13.9} & -21.8 & 14.6 & -66.6 & \underline{-4.7K} & -8.5K & -9.6K & -13.7K
 \\

\cdashline{2-15}

& \multirow{4}{*}{Unified}
& \textsc{T5[MaxEnt]}
& 63.8 & \textbf{74.6} & \textbf{85.3} & 58.3 & 6.0 & \textbf{28.6} & \underline{36.1} & -71.7 & -5.4K & \textbf{-4.8K} & \underline{-9.1K} & -13.6K  \\

& & \textsc{T5[MaxProb]}
& 61.6 & \underline{74.4} & \textbf{85.3} & 56.7 & \textbf{15.3} & \underline{18.1} & \textbf{36.6} & \underline{-18.2} & \textbf{-4.3K} & \underline{-5.9K} & \textbf{-9.0K} & \underline{-7.8K} \\

& & \textsc{T5[FeatMD]}
& 67.5 & 57.1 & 67.6 & 50.1 & -9.1 & -315.3 & 14.1 & \textbf{50.1} & -7.2K & -39.6K & -9.9K & \textbf{50.1}
 \\

& & \textsc{T5[FeatRMD]}
& \underline{72.8} & 55.8 & 76.4 & 49.9 & -48.0 & -352.3 & -153.2 & -296.4 & -11.4K & -43.4K & -42.8K & -36.5K
 \\

\hline
\hline

\cellcolor{white!50} \multirow{7}{*}{API}
& \cellcolor{white!50} \multirow{5}{*}{Pipeline}
& \textsc{CLS$_P$} → \textsc{SQLPrompt}
& \textbf{88.9} & \textbf{88.7} & \textbf{85.3} & 67.1 & -2.5 & -3.2 & -48.0 & -126.5 & -8.6K & -9.7K & -24.8K & -20.3K \\

\cellcolor{white!50} 
& \cellcolor{white!50}  & \textsc{CLS$_P$ → DIN-SQL}
& 61.4 & \underline{75.7} & 61.5 & \textbf{75.0} & -304.1 & -146.6 & -310.6 & \underline{-39.8} & -34.7K & -23.6K & -69.4K & -12.0K
 \\

& & \textsc{CLS$_{P}$} → \textsc{MAC-SQL}
& 73.2 & 71.0 & 66.1 & \underline{74.4} & -169.4 & -198.2 & -260.0 & -46.1 & -23.0K & -28.6K & -60.8K & -12.6K \\

& & \textsc{SQLPrompt} → \textsc{Error$_P$}
& 52.4 & 55.8 & 54.3 & 72.1 & 24.1 & 5.2 & 9.4 & -107.2 & -2.6K & -5.3K & -8.3K & -18.8K \\

& & \textsc{CLS$_P$} → \textsc{SQLPrompt} → \textsc{Error$_P$}
& 54.5 & 58.9 & 57.4 & 67.6 & \textbf{51.4} & \textbf{45.8} & \textbf{46.7} & -41.5 & \textbf{-245.5} & \textbf{-1.3K} & \textbf{-1.9K} & \underline{-11.4K} \\
\cdashline{2-15}

& \multirow{2}{*}{Unified}
& \textsc{SQLPrompt[Demo]}
& \underline{73.4} & 70.4 & 68.6 & 66.8 & -190.2 & -226.1 & -241.3 & -265.3 & -25.0K & -31.5K & -57.8K & -34.9K
 \\

& & \textsc{SQLPrompt[Voting]}
& 66.2 & 67.4 & \underline{73.4} & 50.7 & \underline{41.0} & \underline{40.2} & \underline{45.0} & \textbf{29.8} & \underline{-2.3K} & \underline{-2.8K} & \underline{-5.2K} & \textbf{-2.1K}\\

%\cdashline{2-15}

\hline


\end{tabular}
\end{adjustbox}

\label{tab:main_all}
\end{table*}
